Compositional Generalization Requires Compositional Parsers

A rapidly growing body of research on compositional generalization investigates the ability of a semantic parser to dynamically recombine linguistic elements seen in training into unseen sequences. We present a systematic comparison of sequence-to-sequence models and models guided by compositional principles on the recent COGS corpus (Kim and Linzen, 2020). Though seq2seq models can perform well on lexical tasks, they perform with near-zero accuracy on structural generalization tasks that require novel syntactic structures; this holds true even when they are trained to predict syntax instead of semantics. In contrast, compositional models achieve near-perfect accuracy on structural generalization; we present new results confirming this from the AM parser (Groschwitz et al., 2021). Our findings show structural generalization is a key measure of compositional generalization and requires models that are aware of complex structure.

==> figs/amalgebra.tex <==
\begin{figure}[htb]  % note: can use \fbox{} around tikzpic/forest to have frame
    \captionsetup[sub]{font=small}
    \centering
        %\tiny % smaller fontisze: does is overwrite other definitions?
        \begin{subfigure}[b]{0.33\columnwidth}  %% --Final graph---
        \centering
        %\input{figs/theBoyWantedToGo}
        \begin{tikzpicture}[node distance=30pt,font=\scriptsize]
            \node (want) [nnode, very thick] {want};
            \node (the) [dnode, left of=want, xshift=-10pt] {the};
            \node (boy) [nnode, below of=the] {boy};
            \node (go) [nnode, right of=boy, xshift=10pt] {go};
            % Edges
            \draw [arrow] (want) -- node[anchor=south] {agent} (boy);
            \draw [arrow] (want) -- node[anchor=north] {xcomp} (go); %west
            \draw [arrow] (go) -- node[anchor=north] {agent} (boy);
            \draw [arrow] (the) -- node[anchor=east] {iota} (boy);
        \end{tikzpicture}
        \caption{Final graph}\label{fig:amalgebra:graph}
    \end{subfigure}
    \begin{subfigure}[b]{0.65\columnwidth}  %% ---Constants---
        \centering
        \begin{tikzpicture}[node distance=30pt,font=\scriptsize]
            \node (want) [nnode, very thick] {want};
            \node (want-s) [nnode, below of=want, xshift=-13pt] {$\srcr{S}$};
            \node (want-o) [nnode, below of=want, xshift=+13pt] {$\srcr{O[S]}$};
            \node (go) [nnode, very thick, right of=want, xshift=+10pt] {go};
            \node (go-s) [nnode, below of=go] {$\srcr{S}$};
            \node (boy) [nnode, very thick, right of=go-s, xshift=-5pt] {boy};
            \node (the-m) [nnode, right of=boy, xshift=-5pt] {$\srcr{M}$};
            \node (the) [dnode, very thick, above of=the-m] {the};
            % Edges
            \draw [arrow] (want) -- node[anchor=east] {agent} (want-s);
            \draw [arrow] (want) -- node[anchor=west] {xcomp} (want-o);
            \draw [arrow] (go) -- node[anchor=west] {agent} (go-s);
            \draw [arrow] (the) -- node[anchor=east] {iota} (the-m);
        \end{tikzpicture}
        \caption{Constants $\G{want}$, $\G{go}$, $\G{boy}$, and $\G{the}$}\label{fig:amalgebra:constants}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.43\columnwidth}  %% --AM term---
        \centering
        \begin{center}
        %\resizebox{\linewidth}{!}{
        \begin{forest}
            for tree={align=center, l sep=4pt, l=\baselineskip, s sep=4pt, font=\scriptsize, inner sep=1.5} % l: (parent to child)
            [{\app{\src{S}}}, for tree={fill=colorwant}
                [{\app{\src{O}}}
                    [{\G{want}}]
                    [{\G{go}}, for tree={fill=colorgo}]
                ]
                [{\modify{\src{M}}}, for tree={fill=colorboy}
                    [{\G{boy}}]
                    [{\G{the}}, for tree={fill=colorthe}]
                ]
            ]
        \end{forest}
        %}
        \end{center}
        \caption{AM Term}\label{fig:amalgebra:amterm}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\columnwidth}  %% --AM dep tree---
        %\centering
        \begin{center}
        %\resizebox{\linewidth}{!}{
        \begin{forest} % for tree={.., l sep =0pt, l=\baselineskip} : l-distance between node and its parent
            for tree={draw, align=center, no edge, font=\scriptsize, inner sep=1} % draw nodes with border, draw edges yourself, 
            [parent, phantom
              [{\G{the}\\the}, name=the, fill=colorthe]
              [{\G{boy}\\boy}, name=boy, fill=colorboy]
              [{\G{want}\\wanted}, name=want, fill=colorwant]
              [{$\bot$\\to}, name=to]
              [{\G{go}\\go}, name=go, fill=colorgo]
            ]
            \draw[->] (want) to[out=north, in=80, edge node={node[above, fill=colorwant, font=\scriptsize, inner sep=3] {\app{\src{S}}}}] (boy);
            \draw[->] (want) to[out=60, in=120, edge node={node[above, fill=colorwant, font=\scriptsize, inner sep=3] {\app{\src{O}}}}] (go);
            \draw[->] (boy) to[out=100, in=80, edge node={node[above, fill=colorboy, font=\scriptsize, inner sep=3] {\modify{\src{M}}}}] (the);%pos=0.65,
        \end{forest}
        % }
        \end{center}
        \caption{AM dependency tree}\label{fig:amalgebra:amdeptree}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.45\columnwidth}  %% -- want go (APP)---
        \centering
        \begin{tikzpicture}[node distance=30pt,font=\scriptsize]
            \node (want) [nnode, very thick] {want};
            \node (go) [nnode, below of=want] {go};
            \node (subject) [nnode, left of=go, xshift=-8pt] {$\srcr{S}$};
            % Edges
            \draw [arrow] (want) -- node[anchor=east] {agent} (subject);
            \draw [arrow] (want) -- node[anchor=west] {xcomp} (go);
            \draw [arrow] (go) -- node[anchor=north] {agent} (subject);
        \end{tikzpicture}
        \caption{$\app{\src{O}}\of{\G{want},\G{go}}$}\label{fig:amalgebra:wantGo}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\columnwidth}  %% -- the Boy (MOD) ---
        \centering
        \begin{tikzpicture}[node distance=30pt,font=\scriptsize]
            \node (the) [dnode] {the};
            \node (boy) [nnode, very thick, below of=the] {boy};
            % Edges
            \draw [arrow] (the) -- node[anchor=east] {iota} (boy);
        \end{tikzpicture}
        \caption{$\modify{\src{M}}\of{\G{boy},\G{the}}$}\label{fig:amalgebra:theBoy}
    \end{subfigure}
    %\fbox{\LARGE \todo{Figure should go here}}
    %\includegraphics[scale=.25]{figs/dummyAmAlgebra.png}
    \caption{
        AM analysis for the sentence \sentence{The boy wanted to go},
        slightly adapted from \citet[Fig.~1]{lindemann-etal-2019-compositional}.
        \todo{get spacing right}
    }\label{fig:amalgebra}
\end{figure}

==> halde/background.tex <==
%% Background section
%% - the AM parser and AM algebra
%% - the COGS dataset (Kim & Linzen, 2020)
\section{Compositionality}\label{sec:background}

\subsection{Compositional Generalization}

\ld{a rough first pass; will condense and make more precise once the story is more coherent! see also \href{https://docs.google.com/document/d/1uuIPmM_bShv7eti9J4V_Qlo64a6y0wryHR5QLbdBfmc/edit}{this}}
Basically, compositional generalization is the ability to generalize to new linguistic structures using compositional principles. For humans, this is understood as the algebraic capability to understand and produce a potentially infinite number of novel linguistic expressions by dynamically recombining known elements \citep{chomsky-1957-syntactic,fodor-pylyshyn-1988-connectionism,fodor-lepore-2002-compositionality}. For language models, the task is a semantic parsing task: a language model is expected to construct a semantic representation of a given English sentence. Importantly, the training and evaluation sets for such a task systematically differ such that success on the evaluation set requires out-of-distribution generalization \citep{kim-linzen-2020-cogs}.

It has been argued that the lack of compositionality is one reason why modern neural networks require huge amounts of data to induce correct generalizations, in stark contrast to humans \citep{lake-baroni-2018-generalization}. Robust compositionality requires a theory of syntax, a theory of what meanings are, and a theory of the functions that allow meanings to combine. For example, human grammar accommodates the semantic difference between arguments (\textit{\textbf{The girl} laughs}), restrictive modifiers (\textit{The professor \textbf{of physics} laughs}), and non-restrictive modifiers (\textit{The professor \textbf{under the umbrella} laughs}) with distinct syntax. This reflects the understanding that, in a compositional grammar, both the syntax and semantics are algebras, and there is a homomorphism that maps elements of the syntactic algebra onto elements of the semantic algebra \cite{partee2008compositionality,liu-etal-2021-learning}. 

Much current work on compositional generalization follows the distinction of \citet{kim-linzen-2020-cogs} between \textit{lexical generalization}, a novel combination of a familiar primitive and a familiar structure, and \textit{structural generalization}, a novel combination of two familiar structures such that the sentence structure itself is novel. For example, while simple object to subject NP substitution is considered lexical, CP or PP recursion is considered structural. Though this is a helpful distinction for parsing and evaluation purposes, it glosses over the nuances of compositionality such as PP attachment preference and ambiguity, and word selectional preference based on features like animacy (limitations \citeauthor{kim-linzen-2020-cogs} note themselves). For example, in a sentence such as \textit{The hedgehog loves the girl next to the bear with its whole heart}, the PP attachments are unclear: while the first PP has a slight reading preference for modifying \textit{the girl}, the second PP had a preferred reading for modifying the verb. The most salient reading for a human speaker will depend both on lexical features and context, elements that current tasks dedicated to compositional generalization lack. \ld{K\&L also note the need for constraints on generalization}


\subsection{COGS dataset \citep{kim-linzen-2020-cogs}}\label{subsec:cogsdataset}

\citet{kim-linzen-2020-cogs} introduced the COGS\footnote{
    %COGS stands for \textbf{CO}mpositional \textbf{G}eneralization Challenge based on \textbf{S}emantic Interpretation. 
    %The dataset is publicly available: 
    \url{https://github.com/najoungkim/COGS}.
} 
dataset, a benchmark for compositional generalization, with (sentence, logical form) pairs, e.g.\footnote{
     examples slightly modified for ease of presentation.
}:

% See Table~\ref{tab:cogssamples} for some examples.
% \input{tables/cogs_examples}
\begin{exe}
    \ex\label{ex:boywanted} The boy wanted to go. \\
    \lform{* boy($x_1$) ; want.agent($x_2, x_1$) $\land$ want.xcomp($x_2, x_4$) \\ $\land$ go.agent($x_4, x_1$)}
    \ex\label{ex:other} Ava was lended a cookie in a bottle. \\
    \lform{lend.recipient($x_2,$ Ava) \\ $\land$ lend.theme($x_2, x_4$) \\ $\land$ cookie($x_4$) \\ $\land$ cookie.nmod.in($x_4, x_7$) \\ $\land$ bottle($x_7$)}
    \ex\label{ex:cprec} Ava said that Ben declared that Claire slept. \\
    \lform{say.agent($x_1,$ Ava) \\ $\land$ say.ccomp($x_1, x_4$) \\ $\land$ declare.agent($x_4,$ Ben) \\ $\land$ declare.ccomp($x_4, x_7$) \\ $\land$  sleep.agent($x_7,$ Claire)}
    \ex\label{ex:prim_touch} touch \\
    \lform{$\lambda a. \lambda b. \lambda e.$ touch.agent($e, b$) $\land$ touch.theme($e, a$)}
\end{exe}

% Input
The English declarative sentences on the input side
% \footnote{
%     in contrast to grounded semantic parsing which often uses interrogative sentences (e.g. CFQ of \citet{keysers-etal-2020-measuring}) and in contrast to the much more limited imperatives used in SCAN \citep{lake-baroni-2018-generalization}.
% }
% Output
are mapped to a logical form %(e.g.~\crefrange{ex:boywanted}{ex:prim_touch}) 
which are post-processed forms of \citet{reddy-etal-2017-universal}. Note that they are not grounded in any database.
%\todo{describe logical form syntax with example} % examples should ideally be running examples (for broad overview of logical form things, generalization types (structural, primitive, lexical)
Except for \sortof{primitives} (e.g.~\cref{ex:prim_touch}) which will be discussed below, logical forms consist of a conjunction of terms and a possibly empty list of terms prefixed to this conjunction using iota operators ($\iota$ written as $*$).
A term consist of a predicate name (e.g.~\lform{boy}, \lform{want.agent} or \lform{cookie.nmod.in})
and one or two arguments which are variables (e.g. $x_1, x_2, \dots$ or $a,b,e$ for primitives respectively) or proper names like \lform{Ava}.
The subscript of a $x_i$ variable reveals the alignment to the $i$th input token (0-indexed).
The iota terms are only used for definite NPs like \phrase{the boy} (cf.~\cref{ex:boywanted}).\footnote{
    compare to the indefinite NP \phrase{a cookie} in \cref{ex:other} 
    which is part of the normal conjunction and not the iota prefix.
}
Note that the terms are sorted based on the input token position of their arguments.
%\footnote{but the list of iota terms always fully precedes the conjunction.}
% what about primitives?
This is especially relevant for exact match evaluation.\\
%%Primitive exposure examples (see page 5 in cogs paper and appenxix E.2 page 14)
There are also \emph{primitives} in the training data which represent the \sortof{meaning} of one word in isolation (cf. \cref{ex:prim_touch}). %Required for 'primitive' to X generalization types (5 of the 21 generalization types)
%\todo{show variation of primitives?}% 'Ava' -> \lform{Ava}, 'ball' -> \lform{$\lambda a.$ ball($a$)}, ...
% no OOV words?
For more details we refer the reader to their paper. %\citet{kim-linzen-2020-cogs}.

% Required generalizations
On the generalization set the models are required to make 21 types of generalizations at once.\footnote{
    unlike SCAN of \citet{lake-baroni-2018-generalization}
    with separate sets for each generalization type
} 
This includes
generalizing from a primitive (e.g. \word{shark}) to its usage in context (e.g. \word{a chief heard the shark}), usage of nouns in subject position that were only observed as objects in training (and vice versa),
generalizing to higher CP/PP recursion depths, or generalizing to another verb argument structure (e.g. active vs passive).
% obj pp to subj pp
% verb argument structure alternation: active to passive, object omitted transitive to transitive, double object dative to PP dative
% verb class: e.g. agent np to unaccusative subject
%\todo{mention few generalizations, including lexical and structural}.
%note: no OOV tokens?
For a full list we refer to their paper. % \citep{kim-linzen-2020-cogs}.%specifically Table 1 on p.9089 for an overview and section 3 (p. 9088 to 9091)


\citet[§5.2.1]{kim-linzen-2020-cogs} distinguish between lexical and more structural generalizations\footnote{
    \todo{is structural generalization synonymous to \citet{liu-etal-2021-learning}'s \emph{algebraic recombination}?}
}. 
Most of the 21 generalization types in COGS address lexical generalizations: 
interpreting a word in structure only seen with other words, e.g. using a noun in a grammatical role it hasn't been seen with. The 3 structural generalization types in COGS are not tied to specific words, but require generalization to a novel combination of familiar structures, such as deeper recursion (right-branching PP or CP) or observing a PP modifier at a new grammatical role (object PP to subject PP).
Since the lexical generalization types are overrepresented in COGS, models targeting only or mostly these will look much better at \emph{compositionality} than they actually are: 
\ignore{The large pretrained seq2seq model BART achieved an exact match score of 68 to 71\todo{check numbers}\pw{this will be presented in later sections!}, and}
\citet[Table 2]{akyurek-andreas-2021-lexicon} report that even an LSTM with a copy function can achieve 66\% exact match accuracy and \citet{akyurek-andreas-2021-lexicon}'s more elaborate approaches all focusing on learning a good lexicon worked very well on the lexical cases but failed at structural generalization.
%\todo{other papers as well?}.
% It is exactly the more structural generalizations that are important for what linguists would call \emph{compositionality}.
% Note that unlike for the two recursion generalizations tested, the ObjPP to subjPP generalization type doesn't require the model to generalize to a deeper (constituency tree) structure and/or longer sentence. Still it seems challenging.\todo{mention?}

%In contrast to the train set in which the 143 primitives and 12 exposure examples only appear once, their occurrence count is increased to 100 each to arrive at the train100 set yielding a dataset size of 39,500 samples.
% Exposure examples are full sentences \todo{elaborate}
% they contain a new word (noun/verb, not present in the rest of the training data) which on the generalization set will be seen in a new configuration. E.g. the subject-common noun exposure example is a sentence with \word{hedgehog} as the subject, on the generalization set, however this word is only seen in object position (subject to object common noun generalization type).
% While the primitives are necessary for the 5 generalization types from primitives to their usage in context, the exposure examples are relevant for 13 generalization types, namely the ones which are neither about primitives nor about structural generalizations (recursion and objPP to subjPP).
% Terminology? in the paper they talk about 'primitive exposure examples' at some point
% train:    in_distribution 24,000 primitive    143 exposure_example_*    12   = 24,155
% train100: in_distribution 24,000 primitive 14,300 exposure_example_* 1,200   = 39,500

% Models tested
%\citet{kim-linzen-2020-cogs} report results of standard seq2seq models (Transformer and uni/bi-directional LSTMs) on this dataset (without any pretrained word embeddings): the models perform nearly perfectly on the in distribution test set, but fail dramatically on the generalization set. 
% Evaluation procedure:
%They use exact match accuracy as an evaluation metric, and in the error analysis additionally mention token-level edit distance and well-formedness (missing final closing parenthesis). 


\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.42\textwidth}
    \centering
    %\includegraphics[width=\textwidth]{figs/subj-obj-pp}
    \hbox{\tiny
      \input{figs/tree_to_subj_pp}
    }
    \caption{object PP to subject PP}\label{fig:structural-generalization:toSubjPP}
  \end{subfigure}
  \begin{subfigure}[b]{0.56\textwidth}
      \centering
      %\includegraphics[width=\textwidth]{figs/pp-recursion}
      \hbox{\tiny
        \input{figs/tree_pp_recursion}
      }
      \caption{PP recursion}\label{fig:structural-generalization:PPrecursion}
  \end{subfigure}
  \caption{Structural generalization in COGS. \todo{get spacing right}}
  \label{fig:structural-generalization}
\end{figure*}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> halde/cogs_with_amparser.tex <==

\ld{there should be a transition here explaining how the parser models the syntax/semantics homomorphism discussed in the intro and 2.1., and thus should help us achieve the task at hand}\pw{rewritten a bit, but we never explicitly model true syntax}

% We need to explain
% - apply/modify/am dependency trees
% - graph constants, sources (they are similar to the 'primitives' in COGS): what about type requests?
% - how the parser works: supertagging plus dependency parsing
% - learning source names? 
% - still required supervision: alignments (nodes to tokens) and blob heuristics (put edge into graph constant of which incident node?)
% Ideally we can have running examples like ``The boy wanted to go'', among others
%
% see amparser.bib for references
%  lindemann-etal-2020-fast, donatelli-etal-2020-normalizing, groschwitz-2019-thesis, courcelle-engelfriet-2012-graph, 

Instead of directly predicting a graph, AM dependency parsing predicts graph fragments (so-called \emph{as-graphs}) and dependency structures labelled with operations from the \emph{Apply-Modify algebra} \citep[][AM algebra for short]{groschwitz-etal-2017-constrained} as the compositional structure describing how to combine these fragments. This approach doesn't explicitly model syntax/syntactic algebra, but the semantic dependency structure usually resemble syntactic dependency structures \pw{is this true?}.

\input{figs/amalgebra}
The AM algebra provides two operations to combine graphs: Apply (\app{}) and Modify (\modify{}).
Take for example \cref{fig:amalgebra}:\\
Apply is used to fill an argument, e.g. $\app{\src{O}}\of{\G{want},\G{go}}$ (\cref{fig:amalgebra:wantGo}) means replacing the source \srcr{O} with its argument's graph $\G{go}$, more precisely its root node. Nodes with same sources ($\srcr{S}$ in $\G{want}$ and $\G{go}$) merge.
The $[\srcr{S}]$ at the \srcr{O}-source of \G{want} is a \emph{type request} demanding the argument to have an \srcr{S}-source. If the argument can't fulfill this request, the operation is not allowed and said to be not \emph{well-typed}.\\
Modify is used to add modifiers, e.g. \word{boy} is modified by \word{the}, written as $\modify{\src{M}}\of{\G{boy},\G{the}}$ (\cref{fig:amalgebra:theBoy}): the node with the respective source (e.g. \srcr{M} is merged with the root of the modifiee (\word{boy}). % PW: that the determiner modifies the noun contrasts with certain theories in syntax and semantics (e.g. Generalized Quantifier Theory), but since COGS is lacking adjectives/adverbials one would normally explain modification with, and PPs are a bit special and also length-wise dispreferred (>= 2 extra words), I guess determiners are the only option? 

The graph fragments combined by these operations are so-called \emph{as-graphs}: they each contain exactly one root node (bold outline) and can optionally contain sources (marked in red), e.g. \G{the} contains a \srcr{M}-source.
The type of an as-graph is the set of open sources it contains, e.g. $\G{want}$ has type $\{\srcr{S}, \srcr{O}[\srcr{S}]\}$.
\todo{do we need AM term in (\cref{fig:amalgebra:amterm}) ?}
As-graphs for individual tokens are called \emph{graph constants} (e.g. \cref{fig:amalgebra:constants}).
The \emph{AM dependency tree} (AM dep-tree for short) in \cref{fig:amalgebra:amdeptree} summarizes the compositional structure of the graph it can be deterministically evaluated to (\cref{fig:amalgebra:graph}).
For decomposing a graph into these AM dep-trees, a bit of supervision is needed: node to token alignments are needed and heuristics for assigning edges to either their target or source node. Before \citet{groschwitz-etal-2021-learning}, there were further heuristics needed to decide on source names for nodes. % e.g. for each node with a source, select one including possible requests..
% Question: should our example have 'meaningful' source names (S,O,..) and later we just say 'oh btw, with the unsupervised parser we don't need to specify source names, but let the parser learn them (and just provide how many different sources we want)' ? Cunfusion Tradeoff : uninformative sourcenames vs change from S,O,M to S0,S1,S2 ?
% not explained: result of operation can be used in another round, the notion of AM term

%% The AM parser
% maybe we can even compare learning source names vs using the supervised ones (have to think about how time-consuming it would be to implement edge2source() in the COGSBlobUtils.java and other code that needs to be changed/added.
The \emph{AM parser} \citep{groschwitz-etal-2018-amr} basically consists of a neural (graph-based) dependency parser for the AM dep-tree %\cite{kiperwasser-goldberg-2016-simple}\cite{dozat-manning-2017-deep}
and a supertagger for the graph constants. This problem factorization carries over to \citet{groschwitz-etal-2021-learning}'s use of tree automata to alleviate supervision further by additionally learning source names jointly with the rest. % hence, in the following the sources no longer have syntax-inspired names like \srcr{S}, \srcr{O} or \srcr{M}, but \sortof{meaningless} ones like \srcr{S0}, \srcr{S1} and \srcr{S2}.
AM dependency parsing has been applied to multiple graphbanks including AMR, SDP and EDS \citep{groschwitz-etal-2018-amr,lindemann-etal-2019-compositional, donatelli-etal-2019-saarland},
but so far to no compositional generalization dataset.

%To summarize the AM parser models compositionality by dividing the task of semantic parsing into supertagging (lexicon) and AM dependency parsing (~syntax) with Apply and Modify as the compositional rules.









Logical forms are just provided as strings,
%\footnote{unfortunately no grammar mentioned, but post processed \citet{reddy-etal-2017-universal}},
but since the AM parser and AM algebra operate on graphs, we need to transform the logical forms to graphs first.
We noticed that the logical forms of COGS look quite similar to the LOGIC format of Abstract Meaning Representation \citep[AMR for short:][Fig.~1]{banarescu-etal-2013-abstract} and since the AM parser works well on AMR \citep[cf.][]{groschwitz-etal-2021-learning}, we opted for a graph conversion resembling it.
%We can do so, because the COGS logical forms don't consider scope.
See \Cref{fig:cogsgraph} for an example.


\begin{figure}[t] % use figure* to span both columns
    \centering
    %\input{./figs/theBoyWantedToGo.tex}
    \input{./figs/cogsConversionExample}
    \caption{
        %Logical form to graph conversion for \sentence{The boy wanted to go} (cf.~\cref{ex:boywanted}).
        Logical form to graph conversion for \sentence{Ava wanted to eat a cake on the plate}.
        For illustration only we use node names (the part before the `/') to outline the token alignment.\pw{highly artificial example, not coherent with examples from \cref{subsec:cogsdataset} and AM parser section anymore}
        % in COGS the VP argument of a control verb only ever contains 1 word (the verb)
    }\label{fig:cogsgraph}
\end{figure}

\emph{Arguments} of predicates (e.g. $x_1$, \lform{Ava}) are translated to nodes. 
For each predicate name, the first part (e.g.~\lform{want}, \lform{cake}, \lform{eat}) is taken to be the node label of its first argument.\\
\emph{Binary predicates} (i.e.~terms with 2 arguments) are translated into edges, pointing from their first to their second argument, e.g.~\lform{eat.theme($x_3, x_5$)} is converted to a \graphedge{theme} edge from the \graphnode{eat} node ($x_3$) to the  \graphnode{cake} node ($x_5$),
with exception of preposition-induced predicates.
Preposition meaning \lform{cake.nmod.on($x_5,x_8$)} (\phrase{cake on the plate})) is represented as a node (e.g.~\graphnode{on}) with outgoing edges to the two arguments/nouns (\graphedge{nmod.op1} to \word{cake}, \graphedge{nmod.op2} to \word{plate}).
Each \emph{iota term} \lform{*noun($x_{\text{noun}}$);} is treated as if it was a conjunction of the noun meaning (i.e.~\lform{noun($x_{\text{noun}}$)}) and \sortof{definite determiner meaning} binary predicate \lform{the.iota($x_{\text{the}}, x_{\text{noun}}$)}.
In total there are only 8 different edge labels: \graphedge{agent}, \graphedge{theme}, \graphedge{recipient}, \graphedge{xcomp}, \graphedge{ccomp}, \graphedge{iota} and 2 preposition-introduced edges.\\
The AM parser further requires one node to be the \emph{root node}, which we heuristically select as the node with no incoming edges excluding preposition \pw{and determiner?} nodes. 
For training the AM parser additionally needs \emph{alignments} of the nodes to the input tokens.
Luckily all $x_i$ nodes naturally provide alignments (to the $i$th input token). 
Proper names, determiners and prepositions are aligned using simple heuristics.
All edges \sortof{belong} to the graph constant of the node they originate from.
\pw{just describe primitives in appendix? not important for storyline?}

Note that by encoding the logical form as a graph we get rid of the ordering of the conjuncts. The \sortof{correct} order is restored during postprocessing which in turn is crucial for the exact match accuracy.
More details and examples for the graph conversion can be found in \cref{sec:details_cogs2graph}.







==> halde/discussion.tex <==


%% Note: the following paragraphs could be part of the discussion. 
%% If we don't have enough space, we can shorten them or move them to an appendix section.
\todo{shorten this section: remove or shorten paragraphs or move them to the appendix}

%Dataset is unrealistic, why should I care whether models generalize compositionally? BART performs well in practice...(explainability/trustworthiness, data-thirst of neural models,..)

%How many reentrancies are there in the graphs of COGS? Not that many I guess? More tree like?

\paragraph{Pre-trained language models and compositional generalization.}
Numerous papers \citep{furrer-etal-2020-compositional,oren-etal-2020-improving,gu-etal-2021-beyond-iid,shaw-etal-2021-compositional} observed improvements on compositional generalization by using pretraining data and pretrained language models in particular.
Note however that pre-training on an other (possibly larger) dataset, can lead to spoil(er)ing required generalizations. Furthermore the COGS dataset itself should be enough to succeed on the generalization set \pw{well, \citet{kim-linzen-2020-cogs} mention some doubts}
%Neural models tend to be data-hungry: with compositional generalization we try to test models on their ability to utilize the given data fully: The COGS dataset should be enough to make the required generalizations, no further data should be needed to learn the task/succeed. In a similar vein, data augmentation might help here, but it's not the point to just collect more data to get the models to work, but that they couldn't even fully utilize the data that is available to them
(similar to criticism of \citet{linzen-2020-accelerate}?).
% Shaw et al combine a language model with grammar: claim that language models/non-synthetic dataset are necessary to deal `natural language variation`: we showed with our am-parser (either with or without BERT) that it is possible on a synthetic dataset and unlike shaw et al we use in on all examples
On a very high level our AM parsing models also make use of other data sources (beyond BERT if present), because we copied most hyperparameters from AMR experiments of \citet{groschwitz-etal-2021-learning}.
%Since we mentioned the questionable semantic plausibility of some examples in COGS, we can also ask ourselves whether BART \todo{and BERT?} is confused by some of the examples (similar to humans having a preferred reading that is different from the one actually used in COGS).
% examples from train
% [L1]  A rose was helped by a dog .
% [L13]  A cat disintegrated a girl .
% [L19] A cake was stabbed by Scarlett .
% [L36] A drink was eaten by a child .

\paragraph{Pre/postprocessing.} Unlike the standard seq2seq models, the AM parser doesn't have to invest some of its capacity to learn the \sortof{correct} order of terms (exact match evaluation!), because sorting the terms is a postprocessing step.\footnote{
\citet{guo-etal-2020-poset} suggest that learning a (unnecessary) ordering is detrimental for the performance.
}
%\todo{is this an advantage/disadvantage? how can we keep evaluation fair?}
%\citet{guo-etal-2020-poset} made a similar observation on CFQ of Keysers et al. 2020
% postprocessing: easily done, why should the network have to deal with it? that's more an artifact than part of the semantics
% one can even argue that the sorting makes it easier for the models because it mirrors the input sentence order (like diagonal alignment in MT vs completely distorted)
Moreover, by design of our graph-conversion method, the AM parser can't miss a final closing parenthesis like \citeauthor{kim-linzen-2020-cogs}'s Transformer did sometimes. Also the AM parser has more supervision through making alignments between tokens and the output explicit.
%What is more, unlike other parsers \todo{citations?} the AM parser doesn't learn alignments of nodes to tokens but needs them as input during training. These alignments can be easily extracted from the COGS logical forms based on the $x_i$s and heuristics for proper names, determiners and prepositions.% heuristics: for proper names (each only appears once in a sentence: list.index('Ava')), determiners (index of noun minus 1), prepositions (right after noun1, two positions before noun2).

% \paragraph{Prepositions.} Prepositions seem tricky: (1) effect of representation: to reify or not to reify (2) generalization cases involving prepositions, or rather PPs: PP recursion and objPP to subjPP.

\paragraph{Further limitations of the COGS dataset}
We already discussed the overrepresentation of lexical/shallow generalization, but there are more limitations of this COGS dataset:
First, COGS only deals with declarative sentences and completely lacks phenomena like quantifiers, negation, coordination, relative clauses, adjectives, adverbials among others.
Second, the dataset allows only one reading per sentence and therefore neglects ambiguity: models don't have to deal with word-sense disambiguation (only verb classes/alternations?) or scope ambiguities (lack of quantifiers). 
% There are no syntactic ambiguities either. %(e.g. only strictly right branching recursion for instance)
% no idioms (cogs is fully compositional)
Third, even the semantic plausibility is sometimes lacking.
% So what does it tell us about real-word data? (non-synthetic data)? 
% This was just to test compgen, you don't observe it in iid test sets (see the near perfect test set performance of all models on COGS iid test set), but iid test sets are not everything: trustworthiness, hint that model isn't generalizing they way we would expect it/humans to do it, ...
% See also Shaw et al ('Natural language variation') and Dankers et al (https://arxiv.org/abs/2108.05885 : 'global', synthetic datasets miss WSD and idioms)
% However, sicne the AM parser showed good performance on more 'naturalistic' datasets (e.g. AMR) before and we didn't finetune it so much, we are confident that our approach isn't overfitting/toos-epecialized on the synthetic COGS dataset.

% \paragraph{How does generalization look like in the AM parser?}
% One can ask how the 21 generalization types look like for the AM parser. 
%% S.3.1. Novel Combination of Familiar Primitives and Grammatical Roles  (9 in total)
% For the more \sortof{lexical} generalization tasks (primitive to something, nouns as subject and object) it's basically a known supertag together with an AM dep-tree structure that it was not observed with, but the same delexicalized supertag (and also same type) was observed with this structure before.
%% S.3.4. Verb Argument Structure Alternation   (6)
%% &   S.3.5. Verb Class (3) ---> 9 in total
% PP vs double object datives are interesting: does the structure or supertags even change?
% For the verb-argument structure alternation and verb class generalizations, the parser has to learn that the verb can be used with a different graph constant/supertag too (that has a different, but elsewhere known type and according changes to the AM dep-tree), e.g. \todo{to do} % active <->passive, unaccusative -> transitive, object omitted transitive -> transitive, agent NP -> unaccusative subj
% An interesting case are the PP dative vs double object dative generalizations: In the AM parser both should have the same dependency tree structure and supertags \todo{true? and do we observe this in accuracy?}.
%% S.3.2. Novel Combination Modified Phrases and Grammatical Roles  (1)
%% &   S.3.3. Deeper Recursion  (2)  --> 3 in total
% For the more \sortof{structural} generalizations (object to subject PP, CP and PP recursion) it's about dependency structure, but locally (one dep-edge) everything is already known. In the recursion cases, the chain of \app{}/\modify{} just gets longer. For the object to subject modifying PP, \todo{to do} % haven't seen a MOD operation from a subject-position noun (APPs?), but only for Object position (APPo?).


\paragraph{Dependency structure for generalization.} Compositional generalization is mostly described with composition along phrase structure/constituency trees: \todo{examples: COGS, SCAN use CFG, others}. In contrast, the AM parser uses dependency trees. Although these trees can describe a similar set of string languages than the trees produced by a CFG, the view is a different one: there are less nodes in a tree, no abstract phrase categories such as NPs, VPs (along which one can/is required to generalize) although one can try to find equivalents. %\todo{elaborate on difference between dependency and constituency trees}.

\paragraph{AM parsing specifics that helped for COGS.}
Adding the relative distance encodings to the AM parser helped to solve the low-attachement/right branching PP recursion cases, but the question arises whether it would help on non-synthetic data and especially high-attachement PP recursion too. This remains to be tested.
Similarly choosing the projective Astar decoder instead of the fixed-tree decoder helped to a achieve better results on COGS as all gold trees are projective\footnote{
  note that other approaches targeting compositional generalization might implicitly constrain theirselves to projective trees too by using context-free grammars/constituency trees (e.g.~\citet{liu-etal-2021-learning}).
}, but not all sentences in natural language \pw{what about English in particular?} are projective.



%\subsection{On actual compositionality}\label{sec:actual_compos}
% see also Notes document in Google drive (section about structural generalization )
%\todo{is this now already part of our new introduction? delete this subsection then?}
% reflections on COGS definition of compositional generalization and how the term \emph{compositionality} is used in linguistics instead?

% systematic vs compositional generalization
% tricked by the 'dax' example
% terms: systematicity, productivity, locality, ...
%\todo{also emphasize the point that it's not again a race for higher numbers on a benchmark like the PAID paradigm: just because we obtained high scores doesn't mean we solved the task (cf BART on COGS).}
% also with pretraining: COGS data alone should suffice to solve it. Pretraining data could spoiler generalizations
% maybe compare to criticsm of Dankers et al 2021: https://arxiv.org/abs/2108.05885 (synthetic datasets lack idioms and word sense ambiguity...)



==> halde/experiment.tex <==



\paragraph{Performance is better on train100.}
As expected and in line with \citeauthor{kim-linzen-2020-cogs}'s findings, models generalize better when trained on the larger train100 set compared to the normal train set.
However most papers only report numbers on the smaller training set which requires some sort of one-shot learning for the more lexical generalizations, because the lexical trigger words only appeared once in training.  \todo{concrete numbers? which generalization types benefit?}
%Again emphasizing the data-hungriness of neural models?
The AM parser without pretrained embeddings struggles with this one-shot learning, and the  effect of the random seed on generalization performance is also quite high the smaller train set\todo{numbers}. % although this is a common observation in compgen (in contrast on the dev/test set all models look perfect), we would have expected the compositional AM parser to do better due to its compositional structures.
On the train set the AM parser model without BERT \todo{w and w/o rel?} is even worse than a (non-pretrained) LSTM with a copy function \citet[Table 2: 66\% exact match]{akyurek-andreas-2021-lexicon}.

\paragraph{Effect of pretraining.}
Whereas \citet{tay-etal-2021-pretrained}, BART and the AM parser+BERT use pretraining data, the other models do not. 
%the models of \citet{kim-linzen-2020-cogs,akyurek-andreas-2021-lexicon, conklin-etal-2021-meta,liu-etal-2021-learning, ontanon-etal-2021-making, csordas-etal-2021-devil} and the AM parser without BERT don't use external resources.
We see that pretraining seems to help (AM parser with vs without BERT), especially on the train set (\todo{24} points difference), but less so on the train100 set (\todo{1} point). \todo{check this} \todo{variance reduced too?}
% Reason?: on train we have exposure examples and primitives only once (and then they are only 155 samples compared to 24k others. Generalizing from only one occurence is very hard: if the models would do this we would call this overfitting in other scenarios?
% That pretraining helps with compositional generalization is in line with previous research results (Furrer, Oren, ...
%\todo{what about number of params for BART and \citeauthor{tay-etal-2021-pretrained}?}% fair comparison?
%lso: parameter numbers might differ \todo{comparing param sizes?}.
Even without pretrained embeddings, the AM parser outperforms BART on train100.
\todo{when does a model without pretraining beats a pretrained model?}

%\paragraph{The AM parser without pretraining outperforms even pretrained seq2seq models on train100}
%On train100, the AM parser --even without pretrained embeddings-- outperforms even the pretrained BART model.
%Providing further evidence that the compositionality used by the AM parser helps.
%\todo{present numbers}
%\todo{could partially be the graph conversion too.}
%\todo{what about other people's models?}

\paragraph{Structural generalization is hard for seq2seq models.}
% K&L report structural gen is hard, Akyürek & Andreas also didn't do well on them (but they are excused: they focused on the lexical part anyway), Ontanon et al also didn't do well on them (Table 5, p8)
In line with \citeauthor{kim-linzen-2020-cogs}'s findings, we observe from \cref{tab:semantic_generalization_am} that the structural generalization cases (depth generalization aka CP/PP recursion and obj PP to subj PP) are harder to get right.
By separating results per generalization category we reveal that BART struggles with structural generalization even though it performs respectably overall. The same holds for the models of \citet{akyurek-andreas-2021-lexicon} which aim at improving the lexicon of a seq2seq model.
The structured parsing models tested, the AM parser and the current SOTA model LeAR \citep{liu-etal-2021-learning}, in contrast, struggle way less with structural generalizations.\footnote{\todo{similar picture on the larger train100 set, therefore don't report numbers here?}}
%\input{tables/few_gentype_eval}
%See \Cref{tab:selected_gentype_eval} for the numbers for some selected generalization types \todo{not only structural?}% elaborate on importance of *structural* generlaization here or somewhere else?
\todo{2 categories or the three lexical/shallow/deep?}.\\ %(cf. \cref{tab:syntax generalization} for syntax instead of semantics):

For detailed evaluation results see Appendix~\ref{sec:detailed_evaluation_results}.


\subsubsection{Error analysis}\label{subsec:erroranalysis}
\todo{do we have time/space for error analysis?} 
Similar to what is reported for the seq2seq models in \citet{kim-linzen-2020-cogs}, if it doesn't succeed the AM parser also seems to be very close to the solution in some cases (note that exact match is a very strict metric that doesn't reward partial successes) but fails exactly at the output position where the generalization should take effect.\todo{example needed}. \todo{same for BART?}




==> halde/extensions.tex <==


% we can observe the difference between structured and seq2seq parser mainly lies in structural generalization types. BART completely fails on structural generalization types (5.6\%). 
% Remember that in the unlabeled case, the model only need to output original bracket-annotated source tokens (e.g. \lform{A rose} $\to$ \lform{((A)(rose))}). 
% This suggests that BART cannot even recognize correct syntactic structures in structural generalization types, and thus it is not surprising it cannot solve same types in the semantic level. 
% On the other hand, a structured syntactic parser (e.g. benepar) performs well on such generalization types (99.03\%), which explains why structured semantic parsers generally perform well on structural generalization types. 
% \todo{add analysis for non-struct types?}
% \todo{more discussion on structure vs seq2seq?}
% \todo{add attention visualization if we have space?}





% We first explore hypothesis \ref{it:syngen} by training BART as a syntactic parser on COGS. 
% The syntactic annotations are obtained from original PCFG grammar used to generate COGS \cite{kim-linzen-2020-cogs} with NLTK.
% Similar to the semantic case, BART takes as input plain text but now outputs linearized constituent parse trees rather than semantic meaning representations. 
% To make comparison with a structured syntactic parser, we also experimented with a structured constituency parser of \citet{kitaev-klein-2018-constituency}, which consists of a self-attention encoder and a chart decoder.
% % \todo{maybe need detailed description for neural Berkeley parser.} 
% Results are in Table \ref{tab:syntax generalization}.

% \begin{table}[tbh]
%     \centering
%     \begin{tabular}{llrrr}
%         \toprule
%         & &  struct & non-struct & All\\ \midrule
%         \multirow{2}*{label} & BART  & 1.70\% & 86.99\% & 74.81\%\\
%         ~ & benepar & 99.03\% & 85.87\% & 87.75\% \\
%         % \multirow{2}*{unlabel} & BART & 5.6\% & 94.06\% & 77.14\% \\
%         % ~ & benepar & - & - & - \\
%         unlabel & BART & 5.60\% & 94.06\% & 77.14\% \\
%         \bottomrule
%     \end{tabular} 
%     \caption{Exact match accuracy results for syntactic parsing on generalization set of COGS.
%     % \textit{struct} column denotes the average accuracy for structural generalization types consisting of \textit{cp\_recursion}, \textit{pp\_recursion} and \textit{obj\_pp\_to\_subj\_pp}. 
%     % \textit{non-struct} column denotes average accuracy for other 18 generalization types.
%     % \todo{maybe move definitions to early section.}
%     \textit{benepar} denotes the parser from \citet{kitaev-klein-2018-constituency}. \textit{label}/\textit{unlabel} denotes we train the model to output labeled/unlabeled linearized constituent tree.}
%     \label{tab:syntax generalization}
% \end{table}

% \todo{add analysis}
% From Table \ref{tab:syntax generalization}, we can observe the difference between structured and seq2seq parser mainly lies in structural generalization types. BART completely fails on structural generalization types (5.6\%). 
% Remember that in the unlabeled case, the model only need to output original bracket-annotated source tokens (e.g. \lform{A rose} $\to$ \lform{((A)(rose))}). 
% This suggests that BART cannot even recognize correct syntactic structures in structural generalization types, and thus it is not surprising it cannot solve same types in the semantic level. 
% On the other hand, a structured syntactic parser (e.g. benepar) performs well on such generalization types (99.03\%), which explains why structured semantic parsers generally perform well on structural generalization types. 
% \todo{add analysis for non-struct types?}
% \todo{more discussion on structure vs seq2seq?}
% \todo{add attention visualization if we have space?}





% \begin{table}[tbh]
%     \centering
%     \begin{tabular}{lrrr}
%         \toprule
%         &  struct & non-struct & All\\ \midrule
%         BART  & 4.20\% & 89.90\% & 77.61\% \\
%         +syntax input & 6.30\% & 91.47\% & 79.34\% \\
%         +MTL  & 2.60\% & 90.58\% & 78.01\% \\
%         +AttnMask  & 4.54\% & 90.05\% & 77.83\% \\
%         \bottomrule
%     \end{tabular} 
%     \caption{
%       Exact match accuracy results for semantic parsing on generalization set of COGS.
%     }\label{tab:semantic generalization with syntax}
% \end{table}

Results are shown in Table \ref{tab:semantic generalization with syntax}. 
We can observe all methods only gives very limited improvements, especially for structured generalization types. Multi-task learning have been shown useful in low-resource scenarios in machine translation \cite{currey-heafield-2019-incorporating} but not in our case. 
We consider this is because compositional generalization is different from generalizing from limited data in that the former requires learning syntax first and then interpreting syntactically combined lexical tokens into semantics. 
Thus it may not be enough to only make the model output syntax and semantics together. Modeling the causal relation from syntactic to semantic output may address this.
\todo{better description?}

Self-attention mask is very useful in \cite{kim-etal-2021-improving} on a classification task for compositional generalization but poorly on COGS. 
We consider this comes from the difficulty of generation task compared with classification in \cite{kim-etal-2021-improving}. In their classification task, a source sentence is concatenated with a target meaning representation to be classified as a positive or negative sample.
In our generation task, the model need not only encode syntactic information(e.g. self-attention in encoder), but attend to correct tokens for each decoding step(e.g. cross-attention in decoder). 
Also, \cite{kim-etal-2021-improving} combine self-attention mask with entity cross link (e.g. allow attention between aligned entities in sentence and meaning representation), which we do not use in our task.

There are other methods exploiting syntax in downstream tasks \cite{zhang-etal-2019-syntax-enhanced, glavas-vulic-2021-supervised} such as encoding syntax as dense embedding features. 
Here We leave better exploitation of syntax for compositional generalization for future works. 

% PW: Even with the three approaches to enrich BART with syntax information, the seq2seq model wasn't able succeed at the structural generalization tasks on semantic COGS suggesting that  ...?




==> secs/seq2seq.tex <==
\section{Sequence-to-sequence model on COGS} \label{sec:seq2seq}


\subsection{Syntactic generalization}\label{subsec:seq2seq:syntactic_gen}
We first explore hypothesis \ref{it:syngen} by training BART as a syntactic parser on COGS. 
The syntactic annotations are obtained from original PCFG grammar used to generate COGS \cite{kim-linzen-2020-cogs} with NLTK.
Similar to the semantic case, BART takes as input plain text but now outputs linearized constituent parse trees rather than semantic meaning representations. 
To make comparison with a structured syntactic parser, we also experimented with a structured constituency parser of \citet{kitaev-klein-2018-constituency}, which consists of a self-attention encoder and a chart decoder.
% \todo{maybe need detailed description for neural Berkeley parser.} 
Results are in Table \ref{tab:syntax generalization}.

\begin{table}[tbh]
    \centering
    \begin{tabular}{llrrr}
        \toprule
        & &  struct & non-struct & All\\ \midrule
        \multirow{2}*{label} & BART  & 1.70\% & 86.99\% & 74.81\%\\
        ~ & benepar & 99.03\% & 85.87\% & 87.75\% \\
        % \multirow{2}*{unlabel} & BART & 5.6\% & 94.06\% & 77.14\% \\
        % ~ & benepar & - & - & - \\
        unlabel & BART & 5.60\% & 94.06\% & 77.14\% \\
        \bottomrule
    \end{tabular} 
    \caption{Exact match accuracy results for syntactic parsing on generalization set of COGS.
    % \textit{struct} column denotes the average accuracy for structural generalization types consisting of \textit{cp\_recursion}, \textit{pp\_recursion} and \textit{obj\_pp\_to\_subj\_pp}. 
    % \textit{non-struct} column denotes average accuracy for other 18 generalization types.
    % \todo{maybe move definitions to early section.}
    \textit{benepar} denotes the parser from \citet{kitaev-klein-2018-constituency}. \textit{label}/\textit{unlabel} denotes we train the model to output labeled/unlabeled linearized constituent tree.}
    \label{tab:syntax generalization}
\end{table}

% \todo{add analysis}
From Table \ref{tab:syntax generalization}, we can observe the difference between structured and seq2seq parser mainly lies in structural generalization types. BART completely fails on structural generalization types (5.6\%). 
Remember that in the unlabeled case, the model only need to output original bracket-annotated source tokens (e.g. \lform{A rose} $\to$ \lform{((A)(rose))}). 
This suggests that BART cannot even recognize correct syntactic structures in structural generalization types, and thus it is not surprising it cannot solve same types in the semantic level. 
On the other hand, a structured syntactic parser (e.g. benepar) performs well on such generalization types (99.03\%), which explains why structured semantic parsers generally perform well on structural generalization types. 
\todo{add analysis for non-struct types?}
\todo{more discussion on structure vs seq2seq?}
\todo{add attention visualization if we have space?}
\subsection{Compositional generalization from correct syntax}\label{subsec:seq2seq:semantic_gen_with_syntax}
Given that BART cannot learn syntactic generalization, it is natural to ask whether sequence-to-sequence model can do compositional generalization given the correct syntactic structure (cf. hypothesis \ref{it:semgen_with_syn}). 
In this paper we test this with three popular methods described below to incorporate syntax information into our model. For all methods we use labeled constituent parse tree as syntactic annotations. 

\paragraph{Syntax-enhanced Input} We feed parsed text into the encoder instead of plain text (e.g. \lform{A rose} $\to$ \lform{(NP ({Det} A) ({N} rose))}). 
This method is similar to \cite{li-etal-2017-modeling, currey-heafield-2019-incorporating}, but here we directly make the decoder attend to all source tokens. Here syntactic tokens are used to augment feature representations from encoder.  

\paragraph{Multi-task Learning} We also experiment with multi-task learning setting by inserting a special token in the end of each source sentence (e.g. \lform{A rose} $\to$ \lform{A rose <syn> | A rose <sem>}). 
% The special token denotes which formalism the model should output. 
The model is trained to generate targets with corresponding formalism (e.g. syntax parse tree or semantic meaning representation) given the special token. 
This method is mostly used in natural language generation tasks \cite{sennrich-etal-2016-controlling, currey-heafield-2019-incorporating}. Here we use constituent parsing loss as a regularized loss for semantic parsing task. 

\paragraph{Self-attention Mask} \citet{kim-etal-2021-improving} shows that providing sequential encoder with structure hints helps compositional generalization ability on classification task. Here we also test with their method and use syntax as a mask for self-attention layers in encoder. 
Specifically, each token now is only allowed to attend to its head, children and itself in the parse tree during encoding. 
As suggested by \citet{kim-etal-2021-improving}, this method does not \textit{add} any attention capability but remove non-structured attention edges. 
% We only test with \textit{hard} mask method since it is already useful in \cite{kim-etal-2021-improving}.

\begin{table}[tbh]
    \centering
    \begin{tabular}{lrrr}
        \toprule
        &  struct & non-struct & All\\ \midrule
        BART  & 4.20\% & 89.90\% & 77.61\% \\
        +syntax input & 6.30\% & 91.47\% & 79.34\% \\
        +MTL  & 2.60\% & 90.58\% & 78.01\% \\
        +AttnMask  & 4.54\% & 90.05\% & 77.83\% \\
        \bottomrule
    \end{tabular} 
    \caption{
      Exact match accuracy results for semantic parsing on generalization set of COGS.
    }\label{tab:semantic generalization with syntax}
\end{table}

Results are shown in Table \ref{tab:semantic generalization with syntax}. 
We can observe all methods only gives very limited improvements, especially for structured generalization types. Multi-task learning have been shown useful in low-resource scenarios in machine translation \cite{currey-heafield-2019-incorporating} but not in our case. 
We consider this is because compositional generalization is different from generalizing from limited data in that the former requires learning syntax first and then interpreting syntactically combined lexical tokens into semantics. 
Thus it may not be enough to only make the model output syntax and semantics together. Modeling the causal relation from syntactic to semantic output may address this.
\todo{better description?}

Self-attention mask is very useful in \cite{kim-etal-2021-improving} on a classification task for compositional generalization but poorly on COGS. 
We consider this comes from the difficulty of generation task compared with classification in \cite{kim-etal-2021-improving}. In their classification task, a source sentence is concatenated with a target meaning representation to be classified as a positive or negative sample.
In our generation task, the model need not only encode syntactic information(e.g. self-attention in encoder), but attend to correct tokens for each decoding step(e.g. cross-attention in decoder). 
Also, \cite{kim-etal-2021-improving} combine self-attention mask with entity cross link (e.g. allow attention between aligned entities in sentence and meaning representation), which we do not use in our task.

There are other methods exploiting syntax in downstream tasks \cite{zhang-etal-2019-syntax-enhanced, glavas-vulic-2021-supervised} such as encoding syntax as dense embedding features. 
Here We leave better exploitation of syntax for compositional generalization for future works. 

% PW: Even with the three approaches to enrich BART with syntax information, the seq2seq model wasn't able succeed at the structural generalization tasks on semantic COGS suggesting that  ...?

==> tables/depth_eval.tex <==
\begin{table}[tbh]
    \centering
    \begin{tabular}{lrrr}
        \toprule
         &  All & 3--5 & 6--12\\ \midrule
        K\&L UniLSTM & 0.01 & 0.03 & 0.00 \\
        AM-BERT & 0.82 & 0.993 & 0.74 \\
        AM+BERT & 0.765 & 0.995 & 0.66 \\
        \bottomrule
    \end{tabular} % todo: check that  all = (three-to-five * 3/10 + six-to-twelve * 7/10) 
    \caption{
        Influence of recursion depth (CP+PP) on system performance.
        K\&L UniLSTM is \citet[p. 8]{kim-linzen-2020-cogs}'s best model.
        \todo{\cite{akyurek-andreas-2021-lexicon}? \cite{liu-etal-2021-learning}?}
        \todo{our configuration?}.
        \todo{update numbers}.
        All trained on the normal train set \todo{not train100?}.
    }\label{tab:depth_eval}
\end{table}

==> tables/few_gentype_eval.tex <==
\begin{table*}
      \centering 
      \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
      \setlength{\tabcolsep}{2pt}
      
          \begin{tabular}{llccc|ccc|c|c}
      \toprule
    	             &                 &                \multicolumn{6}{c|}{semantic}                 & \multicolumn{2}{c}{syntactic} \\ \cmidrule(lr){3-8} \cmidrule(l){9-10}
    	              &                &    \amBert    &  \amBert+\dist  &     LeAR     &        Lex:Simple &   BART   & BART+syn  &                      Benepar  &        BART        \\
      Class & Generalization type               &   train100    &   train100    &   train   &            train &  train100   &   train100  &             train100 &      train100      \\
      \midrule
      \structg& objPP to subjPP               &  \asbar{49}   &  \asbar{78}   &  \asbar{93}   &       \asbar{0} &  \asbar{0} & \asbar{0} &          \asbar{84}     &         \asbar{1}          \\
      &CP recursion                  &  \asbar{100}  &  \asbar{100}  & \asbar{100} &           \asbar{0} & \asbar{0}  & \asbar{7} &           \asbar{95}     &         \asbar{4}          \\
      &PP recursion                  &  \asbar{41}   &  \asbar{99}   &  \asbar{99}   &       \asbar{1} &  \asbar{10} & \asbar{8} &      \asbar{98}     &         \asbar{8}          \\
      \midrule
      \propg& primitive to object (proper)  &  \asbar{85}   &  \asbar{94}   & \asbar{93} &              \asbar{66} & \asbar{55} &\asbar{98}  &    \asbar{99}     &         \asbar{97}          \\
      &subject to object (proper)            &  \asbar{90}   &  \asbar{96}   & \asbar{93} &            \asbar{64} &  \asbar{86} &\asbar{95} &    \asbar{100}     &         \asbar{94}          \\
      %&primitive to subject (proper)           &  \asbar{100}  &  \asbar{100}  &  \asbar{100}  &         \asbar{100} &  \asbar{96} &\asbar{100}  &    \asbar{100}     &         \asbar{97}          \\
      \midrule
      \lexg&All 16 other types & \asbar{100}    &   \asbar{100} &   \asbar{100}    &   \asbar{100}    & \asbar{99}  &   \asbar{100}    &   \asbar{100}    &   \asbar{96}    \\
    	\midrule[\heavyrulewidth]
      &Overall                       & \asbar{94} & \asbar{98} &   \asbar{99}   &          \asbar{82} & \asbar{83} &\asbar{86} &    \asbar{99}     &         \asbar{83}    \\ \bottomrule
    \end{tabular}
      
      
      
    % \begin{tabular}{llccc|ccc|c|c}
    %   \toprule
    % 	             &                 &                \multicolumn{6}{c|}{semantic}                 & \multicolumn{2}{c}{syntactic} \\ \cmidrule(l){3-8} \cmidrule(l){9-10}
    % 	              &                &    AM    &  AM+rel  &     LEAR     &        Lex:Simple &   BART   & BART+syn  &                      Benepar  &        BART        \\
    %   Grp & Generalization type               &   train100    &   train100    &   train   &            train &  train100   &   train100  &             train100 &      train100      \\
    %   \midrule
    %   1& objPP to subjPP               &  \asbar{45}   &  \asbar{65}   &  \asbar{89.7}   &       \asbar{0}&  \asbar{0} & \asbar{0.0}&          \asbar{83.7}     &         \asbar{0.5}          \\
    %   &CP recursion                  &  \asbar{100}  &  \asbar{100}  & \asbar{100} &           \asbar{0}& \asbar{0.2}  & \asbar{6.5}&           \asbar{94.9}     &         \asbar{3.7}          \\
    %   &PP recursion                  &  \asbar{39}   &  \asbar{99}   &  \asbar{98.7}   &       \asbar{1}&  \asbar{10.2} & \asbar{7.5} &      \asbar{98.3}     &         \asbar{7.8}          \\
    %   \midrule
    %   2& primitive to object (proper)  &  \asbar{91}   &  \asbar{94}   & \asbar{96} &              \asbar{66}& \asbar{55.2} &\asbar{98.1}  &    \asbar{99.2}     &         \asbar{96.9}          \\
    %   &subject to object (proper)            &  \asbar{99}   &  \asbar{93}   & \asbar{96} &            \asbar{64}&  \asbar{85.7} &\asbar{94.7} &    \asbar{99.6}     &         \asbar{94.4}          \\
    % %   \midrule
    %   &primitive to subject (proper)           &  \asbar{100}  &  \asbar{100}  &  \asbar{100}  &         \asbar{100}&  \asbar{95.5} &\asbar{100.0}  &    \asbar{99.9}     &         \asbar{97.1}          \\
    %   \midrule
      
    % 	obj to subj proper            &  \asbar{100}  &  \asbar{100}  &  \asbar{99}  &           \asbar{100}& \asbar{99}  &\asbar{99.9}&    \asbar{100}     &         \asbar{99.4}          \\
    %   (4) common-noun subjects/objects &  \asbar{100}  &  \asbar{100}  &  \asbar{100}  &         \asbar{99.8}&  \asbar{99} &\asbar{98.6}  &    \asbar{81.3}     &         \asbar{77.9}          \\
    %   unacc to trans                &  \asbar{100}  &  \asbar{100}  & \asbar{100} &              \asbar{100}& \asbar{99}& \asbar{99.9} &    \asbar{100}     &         \asbar{99.5}          \\
    % 	prim to inf arg               &  \asbar{100}  &  \asbar{100}  & \asbar{100}  &           \asbar{100}& \asbar{100}& \asbar{100} &    \asbar{100}     &         \asbar{100}          \\
    %   (2) active/passive            &  \asbar{100}  &  \asbar{100}  & \asbar{100}  &             \asbar{99.5}& \asbar{100}& \asbar{99.9} &    \asbar{100}     &         \asbar{99.6}          \\
    % 	Object-omitted trans to trans &  \asbar{100}  &  \asbar{100}  &  \asbar{100}   &          \asbar{100}& \asbar{99}& \asbar{99.9} &    \asbar{100}     &         \asbar{99.4}          \\
    % 	(2) Ditransitve alternation       &  \asbar{100}  &  \asbar{100}  &  \asbar{99.9}  &      \asbar{99}& \asbar{99} &\asbar{99} &    \asbar{99}     &        \asbar{99}        \\
    % 	(3) Verb class                    &  \asbar{100}  &  \asbar{100}  &  \asbar{100}  &       \asbar{100}& \asbar{99} &\asbar{99} &    \asbar{99}     &         \asbar{99}          \\
      
    %   3&All 15 other types & \asbar{100} & \asbar{100} & \asbar{99.9} & \asbar{99.7} & \asbar{99.3} & \asbar{99.8} & \asbar{99.5} & \asbar{95.4} \\
    % 	\midrule[\heavyrulewidth]
    %   &Overall                       & \asbar{94.0} & \asbar{97.7} &   \asbar{97.7}   &          \asbar{82}& \asbar{82.7} &\asbar{85.9} &    \asbar{98.5}     &         \asbar{82.5}    \\ \bottomrule
    % \end{tabular}
    % }
    
    
    
    
    \caption{Exact match accuracies on the individual generalization types. We have compressed all 16 generalization types of the \lexg class into a single row and report the average accuracy. 
    % See the \cref{sec:detailed_evaluation_results} for AM parser, BART, and LeAR details.
    %   \ak{Perhaps we can just fold all generalization types in class 3 into a single row, which is 99--100 for everyone? Maybe leave ``(2) X to subj proper'' and ``(2) X to obj common'' as separate rows, because we
        % talk about them in the text.} 
        % \yy{I will rerun syntax experiments so those numbers might be changed}
    \pw{old version without additional seq2seq models, see other tables (transposed \cref{tab:selected_gentype_eval_transposed}, appendix version \cref{tab:appendix_selected_gentype_eval})}
    }\label{tab:selected_gentype_eval}
  \end{table*}


  %    	prim to object (common)       &  \asbar{100}  &  \asbar{100}  & \asbar{99} & \asbar{99.8} &    ?     &         ?          \\
%    	subj to obj common            &  \asbar{100}  &  \asbar{100}  &  \asbar{99}  & \asbar{99.8} &    ?     &         ?          \\
%    	obj to subj common            &  \asbar{100}  &  \asbar{100}  &  \asbar{99}  & \asbar{100}  &    ?     &         ?          \\
%    	prim to subj common           &  \asbar{100}  &  \asbar{100}  &  \asbar{99}  & \asbar{100}  &    ?     &         ?          \\
%      active to passive             &  \asbar{100}  &  \asbar{100}  & \asbar{100}  & \asbar{100}  &    ?     &         ?          \\
%    	passive to active             &  \asbar{100}  &  \asbar{100}  & \asbar{100}  & \asbar{100}  &    ?     &         ?          \\

  
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/semanticcogs_categories_eval.tex <==
\begin{table}[tbh]
    \centering
    \small
    \begin{tabular}{lrrl}
        \toprule
         &  struct & non-struct & All\\ \midrule
        LeAR* & \asbar{96.07} & \asbar{99.52} & \asbar{99.02} \\
        AM-BERT rel & \asbar{81.17} & \asbar{60.76} & \asbar{63.67}\stderr{6.61}\\
        AM+BERT rel & \asbar{92.00} & \asbar{67.29} & \asbar{70.76}\stderr{14.88} \\
        AM+BERT & \asbar{68.50} & \asbar{80.32} & \asbar{78.57}\stderr{7.71} \\
        BART & \asbar{00.43} & \asbar{79.68} & \asbar{68.35}  \\
        Lex: Simple & \asbar{00.04} & \asbar{95.89} & \asbar{82.25} \\
        \bottomrule
    \end{tabular} 
    \caption{
    Exact match accuracy results for semantic parsing on generalization set of COGS. \textit{struct} column denotes the average accuracy for structural generalization types consisting of \textit{CP recursion}, \textit{PP recursion} and \textit{object PP to subject PP}. \textit{non-struct} column denotes average accuracy for the rest.
    LeAR \citep{liu-etal-2021-learning} numbers reproduced by running their code \todo{2pts higher!}.
    Lex:Simple is taken from \citet{akyurek-andreas-2021-lexicon}.
    Models trained on train.\todo{update numbers, also change to train100?}\pw{but on  train100 don't have numbers for LeAR (and Lex:Simple)}
    }\label{tab:semantic_generalization_am}
\end{table}

==> tables/semanticcogs_main_eval.tex <==
{
%%    \renewcommand*{\thefootnote}{\alph{footnote}} % I want to have
%%    superscript 'a' instead of superscript '1' for a footnote:
%%    superscript with number can be confused with exponentiation when
%%    put after numbers
  %%%  AK: I really don't, especially if all other footnotes are
  %%%  arabic numbers.
\begin{table*}[tbh]
\small
    \centering
    \begin{tabular}{@{}llrrrr@{}} \toprule
%      \renewcommand*{\thefootnote}{\arabic{footnote}}
      && \multicolumn{2}{c}{train} & \multicolumn{2}{c}{train100} \\
      \cmidrule(l){3-4} \cmidrule(l){5-6}
      && Test & Gen & Test & Gen \\ \midrule
      \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{seq-to-seq}}}
      &\citet{kim-linzen-2020-cogs}: Transformer & \oldNumber{96} & \oldNumber{35} & \oldNumber{94} & \oldNumber{63} \\
      &\citet{conklin-etal-2021-meta}: Transformer w. Tree-MAML & \oldNumber{99} & \oldNumber{66.7} & 99 & 74.8 \\
    %   &\citet{ontanon-etal-2021-making}: Transformer tagging  & - & \oldNumber{78.4} & - & - \\ % tagging is not seq2seq, their true seq2seq models perform rather poorly
      &\citet{csordas-etal-2021-devil}: Transformer relative pos. & \oldNumber{100} & \oldNumber{81} & - & 75.7 \\
      &\citet{akyurek-andreas-2021-lexicon}: LSTM + Lex: Simple: Soft & - & \oldNumber{83} & 99 & 84.5 \\
      %&\citet{jambor-bahdanau-2021-lagr}: LAGr (not seq2seq) & ? & \oldNumber{81.5} & - & - \\ % does it even fit in our dichotomy of seq2seq vs compositional?
      %&\citet{zheng-lapata-2021-disentangled}: Transformer (rel) + Dangle $\dagger$& - & \oldNumber{85.8} & - & - \\ % seq2seq architecture but reencode input+output so far for every decoding step : they say without pretraining, but then in results 4.3 section say they use Glove embeddings (so they clearly have access to data beyond cogs?)
      &\citet{zheng-lapata-2021-disentangled}: Roberta + Dangle$^\dagger$ \pw{new} & - & \oldNumber{87.9} & - & - \\ % seq2seq architecture but reencode input+output so far for every decoding step
      &\citet{orhan-2021-compgen}: Transformer mT5 xl $^\dagger$ \pw{new} & - & \oldNumber{84.6} & - & - \\
      &\citet{tay-etal-2021-pretrained}: Transformer  $^\dagger$ & \oldNumber{95} & \oldNumber{77.5} & - & -
      \\
      \cmidrule(l){2-6}
      &BART  $^\dagger$ & 100 & 77.5\stderr{0.4}  & 100 & 82.7\stderr{1.4} \\
      &BART+syn  $^\dagger$ & 100 & 80.2\stderr{0.4}  & 100 & 85.9\stderr{0.3} \\
      \midrule
      %
      %
      \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{compositional}}}      
      &\citet{liu-etal-2021-learning}: LeAR\protect\footnotemark & - & \textbf{98.9}\stderr{0.9} & - & - \\
      \cmidrule(l){2-6}
      &\amToken & 100 & 59.9\stderr{\hspace{.5em}2.7} & 100 & 91.1\stderr{2.3} \\ 
      &\amToken+\dist & 100 & 62.6\stderr{10.8} & 100 & 88.6\stderr{4.9}\\
      &\amBert  $^\dagger$ & 100 & 79.6\stderr{\hspace{.5em}6.4} & 100 & 93.6\stderr{1.4} \\
      &\amBert+\dist  $^\dagger$ & 100 & 78.3\stderr{22.9} & 100 & \textbf{98.4}\stderr{0.9} \\
      \bottomrule
    \end{tabular}
    \caption{
      Exact match accuracies on COGS. Results in gray are taken from the respective papers. $^\dagger$) models that use pretraining. 
    %   \ak{Someone please double-check this.}
        % \yy{exclude \citeauthor{ontanon-etal-2021-making}? see chat?}
    %   after training on train or train100,  
    % evaluated on test and generalization set. 
    % best reported from 
    % \citet{kim-linzen-2020-cogs},
    % \citet[§5.8]{tay-etal-2021-pretrained}, %only 2 numbers reported
    % \citet[Table 5]{ontanon-etal-2021-making}: tagging rel-eb small-2s attention,
    % \citet[Table 3]{csordas-etal-2021-devil}: Transformer w/ relative positions,
    % \citet[Table 2 and 5]{akyurek-andreas-2021-lexicon},
    % \citet[Table 3]{conklin-etal-2021-meta}, and
    % \citet[Table 4]{liu-etal-2021-learning}.
    % \todo{update and check numbers}.
    % Note that some models (bottom) use pretraining.
    % Exact match accuracy is used as an evaluation shown.
    }\label{tab:results}
  \end{table*}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/summary_eval.tex <==
\begin{table}[tbh]
    \centering
    \small
    \begin{tabular}{lrrrr}
        \toprule
                & \multicolumn{2}{c}{COGS syntax} & \multicolumn{2}{c}{COGS semantics} \\ \cmidrule(l){2-3} \cmidrule(l){4-5}
        model           & struct & non-struct & struct & non-struct  \\ \midrule
        BART            & 1.7   & 86.99   & 0.4 & 79.68 \\
        BART+syntax & ?   & ? & ? & ? \\
        benepar & 99.03   & 85.87  & -    & - \\
        AM parser       & -      & -     & 92.00 & 67.29 \\
        \bottomrule
    \end{tabular}
    \caption{
        Summarizing our evaluation results. \textit{COGS syntax} refers to predicting syntactic parse trees, \textit{COGS semantics} to predicting semantics/logical forms on the generalization set.
        AM parser results with BERT embeddings and relative distance encodings.
        Generalization set accuracies after training on \todo{train? not train100?}. \todo{small font used?}
    }\label{tab:summary}
\end{table}
